EnhancePPG: Improving PPG-based Heart Rate Estimation with Self-Supervision and Augmentation

Heart rate (HR) estimation from photoplethysmography (PPG) signals is a key feature of modern wearable devices for health and wellness monitoring. While deep learning models show promise, their performance relies on the availability of large datasets. We present EnhancePPG, a method that enhances state-of-the-art models by integrating self-supervised learning with data augmentation (DA). Our approach combines self-supervised pre-training with DA, allowing the model to learn more generalizable features, without needing more labelled data. Inspired by a U-Net-like autoencoder architecture, we utilize unsupervised PPG signal reconstruction, taking advantage of large amounts of unlabeled data during the pre-training phase combined with data augmentation, to improve state-of-the-art models' performance. Thanks to our approach and minimal modification to the state-of-the-art model, we improve the best HR estimation by 12.2%, lowering from 4.03 Beats-Per-Minute (BPM) to 3.54 BPM the error on PPG-DaLiA. Importantly, our EnhancePPG approach focuses exclusively on the training of the selected deep learning model, without significantly increasing its inference latency

==> tables/data_augmentation.tex <==
\begin{table}[h]
\centering
\caption{DA configurations explored}
\label{tab:da_config}
\begin{tabular}{c|l|c}
\hline
\textbf{Augmentation [x]} & \textbf{Augmentation Type} & \textbf{Percentage (\%)} \\ \hline
\multirow{6}{*}{\textbf{8x}} & Jittering & 100\% \\ 
                             & Scaling & 100\% \\
                             & Time Warping & 100\% \\
                             & Magnitude Warping & 100\% \\
                             & Divide\_2 & 100\% \\
                             & Multiply\_[1.4 - 2, 0.6] & 200\% \\ \hline
\multirow{2}{*}{\textbf{11x}} & Divide\_2 & 100\% \\
                              & Multiply\_[1.2 - 2, 0.1] & 900\% \\ \hline

\end{tabular}
\end{table}
